Online Production Validation in a HEP environment

Petabytes of data are to be processed and stored requiring millions of CPU-years in high energy particle (HEP) physics event simulation. This enormous demand is handled in worldwide distributed computing centers as part of the LHC computing grid. These significant resources require a high quality and efficient production and the early detection of potential errors. In this article we present novel monitoring techniques in a Grid environment to collect quality measures during job execution. This allows online assessment of data quality information to avoid configuration errors or inappropriate settings of simulation parameters and therefore is able to save time and resources.

==> svn.tex <==
{\small $Id: svn.tex 27 2015-09-20 16:07:33Z volkmer@PLEIADES.UNI-WUPPERTAL.DE $} %do beforehand: svn propset svn:keywords "Id" svn.tex


